Detection and Mitigation of Attacks on Transportation Networks as a Multi-Stage Security Game

In recent years, state-of-the-art traffic-control devices have evolved from standalone hardware to networked smart devices. Smart traffic control enables operators to decrease traffic congestion and environmental impact by acquiring real-time traffic data and changing traffic signals from fixed to adaptive schedules. However, these capabilities have inadvertently exposed traffic control to a wide range of cyber-attacks, which adversaries can easily mount through wireless networks or even through the Internet. Indeed, recent studies have found that a large number of traffic signals that are deployed in practice suffer from exploitable vulnerabilities, which adversaries may use to take control of the devices. Thanks to the hardware-based failsafes that most devices employ, adversaries cannot cause traffic accidents directly by setting compromised signals to dangerous configurations. Nonetheless, an adversary could cause disastrous traffic congestion by changing the schedule of compromised traffic signals, thereby effectively crippling the transportation network. To provide theoretical foundations for the protection of transportation networks from these attacks, we introduce a game-theoretic model of launching, detecting, and mitigating attacks that tamper with traffic-signal schedules. We show that finding optimal strategies is a computationally challenging problem, and we propose efficient heuristic algorithms for finding near optimal strategies. We also introduce a Gaussian-process based anomaly detector, which can alert operators to ongoing attacks. Finally, we evaluate our algorithms and the proposed detector using numerical experiments based on the SUMO traffic simulator.

==> prelim.tex <==
\section{Traffic Model}
\label{sec:prelim}

%We begin by providing a brief overview of cell-transmission traffic model and Gaussian processes, on which our game-theoretic model and anomaly-based attack detector are based.

%\subsection{Traffic Model}

To model how traffic flows through a transportation network, we use Daganzo's cell transmission model. % for transportation networks.
Here, we provide a brief summary of this traffic model;
for a more detailed discussion, we refer the reader to~\cite{daganzo1994cell,daganzo1995cell,ziliaskopoulos2000linear}.
\footnote{For readers who are familiar with the cell-transmission model, we recommend to continue with the next section.}
% is primarily based on the work of Ziliaskopoulos~\cite{ziliaskopoulos2000linear}.
For a list of symbols used in the traffic model, see Table~\ref{tab:symbols_traffic}.

\begin{table}[h]
\caption{List of Symbols from the Traffic Model}
\label{tab:symbols_traffic}
\centering
\renewcommand*{\arraystretch}{1.0}
\setlength{\tabcolsep}{3pt}
\begin{tabular}{| c | p{10.25cm} |}
\hline
Symbol & \multicolumn{1}{l|}{Description} \\
\hline
\multicolumn{2}{|c|}{Cell Transmission Model} \\
\hline
$x_i^t$ & number of vehicles in cell $i$ at time $t$ \\ 
\rowcolor{Gray} $y_{ij}^t$ & number of vehicles moving from cell $i$ to cell~$j$ at time~$t$ \\
$Q_i^t$ & maximum number of vehicles that can flow into or out of cell $i$ during time interval~$t$ \\
\rowcolor{Gray} $\delta_i^t$ & ratio between free-flow speed and backward propagation speed of cell $i$ at time~$t$ \\
$N_i^t$ & maximum number of vehicles in cell $i$ at time~$t$ \\
\rowcolor{Gray} $\Gamma(i)$ & set of successor cells to cell $i$ \\
$\Gamma^{-1}(i)$ & set of predecessor cells to cell $i$ \\
\rowcolor{Gray} $d_i^t$ & demand (inflow) at source cell $i$ during time interval $t$ \\
\hline
\multicolumn{2}{|c|}{Signalized Intersection Model} \\
\hline
$p_{ki}^t$ & inflow proportion from cell $k$ to signalized intersection $i$ \\
\rowcolor{Gray} $\calI$ & set of signalized intersections \\
\hline
\end{tabular}
\end{table}

In the cell transmission model, a road network is divided into \emph{cells}, which represent homogeneous road segments, and time is divided into uniform \emph{intervals}.
The length of a road segment corresponding to a cell is equal to the distance traveled in light traffic by a typical vehicle in one time interval.
Each cell $i$ has three sets of parameters:
\begin{itemize}
\item $N_i^t$ is the maximum number of vehicles that can be present in cell $i$ at time $t$,
\item $Q_i^t$ is the maximum number of vehicles that can flow into or out of cell $i$ during time interval~$t$,
\item and $\delta_i^t$ is the ratio between the free-flow speed and the backward propagation speed of cell $i$ at time $t$ (see~\cite{ziliaskopoulos2000linear} for a detailed explanation).
This constant is used to quantify how the speed of traffic decreases as the cell becomes congested, and can model traffic phenomena such as shockwaves. %For more details, we refer the reader to~\cite{ziliaskopoulos2000linear} and~\cite{daganzo1994cell}.
\end{itemize}

Every cell is connected to one or more other cells: cells that correspond to consecutive road segments or road segments that are joined by an intersection are connected.
The set of cells from which vehicles can move into cell $i$ is called the set of \emph{predecessor cells}, denoted by $\Gamma^{-1}(i)$;
similarly, the set of cells to which vehicles can move from cell $i$ is called the set of \emph{successor cells}, denoted by~$\Gamma(i)$.

At a given time $t$, the state of the transportation network is modeled by the vector $\vx^t$, where the value $x_i^t$ is the number of vehicles in cell $i$.
The traffic model defines how the state of the network $\vx^t$ evolves over time from an initial state $\vx^0 = (0, \ldots, 0)'$.
In each time interval, for every pair of connected cells $i$ and $k$, the number of vehicles $y_{ik}^t$ moving from cell $i$ to cell $k$ is determined by the state of both cells (see below).

Based on their connections, the cells can be divided into five types: ordinary cells, diverging cells, merging cells, source cells, and sink cells.
Next, we describe how the state $x_i^t$ of each cell $i$ evolves.

\paragraph{Ordinary Cells}
Ordinary cells have only one successor cell and one predecessor cell.
For every ordinary cell $i$ and time interval $t$, the state evolves as follows:
\begin{equation}
\label{eq:ordinaryStateEquation}
x_i^t = x_i^{t - 1} + y_{ki}^{t - 1} - y_{ij}^{t - 1} ,
\end{equation}
where $k \in \Gamma^{-1}(i)$ and $j \in \Gamma(i)$ (note that since cell $i$ is ordinary, $k$ and $j$ are uniquely defined).

The flow $y_{ki}^t$ between ordinary cells $k$ and $i$ is
\begin{equation}
y_{ki}^t = \min\{x_k^t,~ \min\{Q_i^t, Q_k^t\},~ \delta_i^t(N_i^t - x_i^t)\} .
\end{equation}
According to the above equation, the flow is limited by three terms:
\begin{itemize}
\item $x_k^t$ since the number of vehicles leaving cell $k$ cannot be greater than the number of vehicles present in cell $k$;
\item $Q_i^t$ and $Q_k^t$ by definition;
\item and $\delta_i^t(N_i^t - x_i^t)$, which limits the flow as cell $i$ becomes congested.
\end{itemize}
By setting $y_{ki}^t$ equal to the minimum of these terms, we assume that drivers do not stop without a traffic reason (until they reach their destination).

\paragraph{Diverging Cells}
Diverging cells differ from ordinary cells in that they have multiple successor cells.
For every diverging cell $i$ and time interval $t$,
\begin{equation}
x_i^t = x_i^{t - 1} + y_{ki}^{t - 1} - \sum_{j \in \Gamma(i)} y_{ij}^{t - 1} ,
\end{equation}
where $k \in \Gamma^{-1}(i)$ (note that since cell $i$ is diverging, $k$ is unique).

The inflow $y_{ki}^t$ is the same as in the case of ordinary cells.
The outflows $y_{ij}^t$ are subject to the following constraints: % determined by the following linear program:
%\begin{equation}
%\max \sum_{j \in \Gamma(i)} y_{ij}^t
%\end{equation}
%subject to
\begin{align}
\forall j \in \Gamma(i): ~ y_{ij}^t &\leq \min\left( Q_j^t,~ \delta_j^t (N_j^t - x_j^t) \right) \\
\sum_{j \in \Gamma(i)} y_{ij}^t &\leq \min\left( x_i^t,~ Q_i^t \right).
\end{align}
Notice that these constraints are analogous to the ones for ordinary cells, with the exception that the limits posed by $x_i^t$ and $Q_i^t$ apply to the sums of the outflows.

\paragraph{Merging Cells}
Merging cells differ from ordinary cells in that they have multiple predecessor cells.
For every merging cell $i$ and time interval $t$,
\begin{equation}
x_i^t = x_i^{t - 1} + \left( \sum_{k \in \Gamma^{-1}(i)} y_{ki}^{t - 1} \right) - y_{ij}^{t - 1} ,
\end{equation}
where $j \in \Gamma(i)$ (note that since cell $i$ is merging, $j$ is unique).

The outflow $y_{ij}^t$ is the same as in the case of ordinary cells.
The inflows $y_{ki}^t$ are subject to the following constraints: % determined by the following linear program:
%\begin{equation}
%\max \sum_{k \in \Gamma^{-1}(i)} y_{ki}^t
%\end{equation}
%subject to
\begin{align}
\forall k \in \Gamma^{-1}(i): ~ y_{ki}^t &\leq \min\left( x_k^t,~ Q_k^t \right) \\
\sum_{k \in \Gamma^{-1}(i)} y_{ki}^t &\leq \min\left( Q_i^t,~ \delta_i^t (N_i^t - x_i^t) \right) .
\end{align}
Again, notice that these constraints are natural extensions of the ones for ordinary cells, except that the limits posed by $Q_i^t$ and $\delta_i^t (N_i^t - x_i^t)$ apply to the sums of the inflows.

\paragraph{Sink and Source Cells}
Sink cells have infinite capacity and allow infinite input flows (i.e., $N_i^t = \infty$ and $Q_i^t = \infty$ for every sink cell~$i$ and time interval $t$); hence, the input flow of sink cell~$i$ is $y_{ki}^t = \min\{x_k^t, Q_k^t\}$. % are determined solely by the state and characteristics of their predecessor cells.

Source cells have infinite capacity but allow only finite output flows (i.e., $N_i^t = \infty$ for every source cell $i$ and time interval $t$).
For every source cell $i$ and time interval~$t$,
%\begin{equation}
$x_i^t = x_i^{t - 1} + d_i^{t - 1} - y_{ij}^{t - 1}$,
%\end{equation}
where $j \in \Gamma(i)$ (note that $j$ is unique) and $d_i^t$ is the demand (inflow) at cell $i$ in time interval $t$ (i.e., $d_i^t$ is the number of vehicles entering traffic at cell $i$ in time interval $t$).


\subsection{Signalized Intersections}

To account for signal control at intersections, we follow Daganzo's proposition~\cite{daganzo1995cell} and introduce the time-dependent parameter $p_{ki}^t$ controlling the inflow proportions of merging cells.
Then, for every signalized merging cell $i \in \calI$ and time interval $t$, the inflows must also satisfy
\begin{align}
\forall k \in \Gamma^{-1}(i): ~ y_{ki}^t &\leq p_{ki}^t Q_i^t \\
\forall k \in \Gamma^{-1}(i): ~ y_{ki}^t &\leq p_{ki}^t \delta_i^t (N_i^t - x_i^t) ,
\label{eq:signalizedIntersectionFlow}
\end{align}
where $\sum_{k \in \Gamma^{-1}(i)} p_{ki}^t = 1$.


\subsection{Solving the Traffic Model}
\label{sec:traffic_solution}

In order to solve the traffic model, that is, to find~$\vx^t$ for every $t > 0$, we use Ziliaskopoulos's linear programming approach~\cite{ziliaskopoulos2000linear}, and formulate the following program:
\begin{equation}
\min \sum_t \sum_i x_i^t
\end{equation}
subject to
Equations~\eqref{eq:ordinaryStateEquation} to~\eqref{eq:signalizedIntersectionFlow},
where $x_i^t \in \Real_{\geq 0}$ for every time $t > 0$ and cell $i$, $y_{ki}^t \in \Real_{\geq 0}$ for every time $t > 0$ and connected cells $k$ and $i$, and the number of time intervals is chosen so that $\vx^t$ reaches $(0, \ldots, 0)$ by the last time interval. 
Note that we assume fractional $x_i^t$ values, since we are interested in a macro solution, not individual vehicles.

Now, observe that the objective of the above linear program is the sum of the number of vehicles traveling (i.e., number of vehicles on the road) over time, which is clearly equal to the \emph{total travel time} of all the vehicles.
In other words, the above solution assumes that vehicles will travel efficiently (i.e., in a way that minimizes their travel time) given that they have to abide the constraints of the traffic model, including the inflow proportions dictated by the traffic signals.
As a consequence, we can use the value of the above linear program---which can be computed efficiently for a given instance---as a measure of network congestion.



